Continuous Pupillography: A Case for Visual Health Ecosystem

This article aims to cover pupillography, and its potential use in a number of ophthalmological diagnostic applications in biomedical space. With the ever-increasing incorporation of technology within our daily lives and an ever-growing active research into smart devices and technologies, we try to make a case for a health ecosystem that revolves around continuous eye monitoring. We tend to summarize the design constraints & requirements for an IoT-based continuous pupil detection system, with an attempt at developing a pipeline for wearable pupillographic device, while comparing two compact mini-camera modules currently available in the market. We use a light algorithm that can be directly adopted to current micro-controllers, and share our results for different lighting conditions, and scenarios. Lastly, we present our findings, along with an analysis on the challenges faced and a way ahead towards successfully building this ecosystem.

==> report_files/IoT_101.tex <==
The Internet of Things, in itself, covers a broad spectrum of topics and devices. The field emerged from a number of overlapping trends ranging from cheap sensors, high compute powers, miniaturization of design, accurate location positioning systems to increased and enhanced and inexpensive network access, and widespread use to mobile phones as interface devices. The devices included in a connected IoT space do not correspond to multi-use computation resources such as phones, tablets or laptops. Instead, they refer to products built for a narrow range of utility and they have the ability to articulate one or all of the three behaviours, which are key to any IoT device: \textbf{sense, analyze and communicate}

The space of IoT is an ever-growing field, and recently enough, the industry is booming with plenty of newer \& smarter applications and use-cases. This increase in IoT trend correlated with a range of different predictions as to how many devices are there in the world and how many more of IoT devices are coming our way. IBM forecasted in 2012 that there would be one trillion such connected devices in 2015 \cite{iwata2012making}, however this still awaits to come true. Cisco anticipated 50 billion devices by 2020, which is one of their widely used predictions \cite{evans2011internet}. Gartner Research's often cited analysis claimed to have 8.4 billion devices in 2017 and anticipated a further increase to 20 billion in 2020 \cite{Gartner17}. Statista recently predicted there would be around 75 billion device market in 2025 \cite{statista2018internet}. However, these predictions ought to be taken with a grain of salt, since it's not always clear as to what is actually included in these analysis; whether mobile phones, tablets are part of it or even if there is a distinction between IP-based and non IP-based devices. This makes it very hard to pinpoint the exact number of such devices now or even in the future. 

\begin{figure}[h]
  \centering
  \includegraphics[width=\linewidth]{picture_references/Examples of IoT (paper 4).png}
  \caption{Consumer \& Enterprise based IoT Examples. \cite{rosner2018privacy}}
  \Description{A number of IoT examples in the domestic and industrial environment }
  \label{fig:IoT_examples}
\end{figure}

Regardless of these changing predictions and definitions, the concept of IoT is a very useful one given the socio-economic impacts of a connected global world. As illustrated in the above example, IoT has a huge potential in improving our daily lives, health outcomes, travelling safety, increased free-time at home through task automation, richer entertainment experiences, making industrial processes efficient and cheaper, and let ourselves know us better. 

However, these changes will come at the expense of more and more audio-visual sensors, cameras, thermal detectors, facial recognition and identification technology, and a handful of personally identifiable stuff. As we get to know ourselves better, and enhance our society's collective experiences of life, we also lead ourselves to a vulnerable and exposed state. In this paper, we tend to discover how these connected devices and the classical notions of private spaces overlap, and what efforts are being made to make it an enjoyable experience, rather than a scary techno-hack movie. 



==> report_files/privacy_definition_model.tex <==
Considering the very broad and diverse spectrum of IoT devices, literature offers many definitions and perspectives related to privacy, with the \textit{information privacy} at the forefront of them all. It was defined by Westin in 1968 as "the right to select what personal information about me is known to what people". Although this definition, which referred to non-electronic devices, is still valid, it is at the same time too generic to enable any focused analysis of the topic. Hence, for the paper, we adopt a definition and reference model used in \cite{ziegeldorf2014privacy} for a more detailed approach:\newline

\textit{Privacy in the Internet of Things is the threefold guarantee to the subject for}
\begin{itemize}
    \item \textit{ awareness of privacy risks imposed by smart things and services surrounding the data subject }
    \item \textit{ individual control over the collection and processing of personal information by the surrounding smart things }
    \item \textit{ awareness and control of subsequent use and dissemination of personal information by those entities to any entity outside the subject’s personal control sphere }
\end{itemize}

The IoT reference model that \cite{ziegeldorf2014privacy} refers to is based on the ITU \cite{union2005internet} and IERC \cite{vermesan2011internet} visions of the IoT and can be summarized as: \textit{Anyone and anything is interconnected anywhere at any time via any network participating in any service}. This reference model describes the entities and information flows of IoT applications. 

\begin{figure}[h]
  \centering
  \includegraphics[width=\linewidth]{picture_references/Overall IoT Scheme (Paper 10).png}
  \caption{IoT Constitution: Sensing, Analyzing and Communicating . \cite{ziegeldorf2014privacy}}
  \Description{IoT Constitution: Sensing, Analyzing and Communicating}
  \label{fig:IoT_module}
\end{figure}

In the model \textbf{four main types of entities} are under consideration as depicted in Figure. \ref{fig:IoT_module}. \textbf{\textit{Smart things}} are everyday things augmented with information and communication technology (ICT), with the ability to collect, process and communicate data about themselves and their environment with other things and humans. Backends host \textbf{\textit{services}} that gather, combine and analyze data from many smart things to offer a value-addition service to the end-user. Humans have two different roles here: either \textbf{\textit{subject}} to data collection by the smart things or \textbf{\textit{recipients}} of data or services. Finally, smart things are connected to services via an \textbf{\textit{infrastructure}} with different characteristics ranging from low-power lossy networks to powerful Internet backbones possibly traversing different intermediate gateways and servers, e.g. firewalls and protocol bridges.

This model abstracts most of the device specific details, interconnection methods and services, and hence provides a high-level overview of the wide range of IoT systems and applications. Though it might not hold true for every scenario, but it does convey a broader sense of the interconnections of IoT in our daily life.  

